Towards Lossless Dataset Distillation via Difficulty-Aligned Trajectory Matching

The ultimate goal of Dataset Distillation is to synthesize a small synthetic dataset such that a model trained on this synthetic set will perform equally well as a model trained on the full, real dataset. Until now, no method of Dataset Distillation has reached this completely lossless goal, in part due to the fact that previous methods only remain effective when the total number of synthetic samples is extremely small. Since only so much information can be contained in such a small number of samples, it seems that to achieve truly loss dataset distillation, we must develop a distillation method that remains effective as the size of the synthetic dataset grows. In this work, we present such an algorithm and elucidate why existing methods fail to generate larger, high-quality synthetic sets. Current state-of-the-art methods rely on trajectory-matching, or optimizing the synthetic data to induce similar long-term training dynamics as the real data. We empirically find that the training stage of the trajectories we choose to match (i.e., early or late) greatly affects the effectiveness of the distilled dataset. Specifically, early trajectories (where the teacher network learns easy patterns) work well for a low-cardinality synthetic set since there are fewer examples wherein to distribute the necessary information. Conversely, late trajectories (where the teacher network learns hard patterns) provide better signals for larger synthetic sets since there are now enough samples to represent the necessary complex patterns. Based on our findings, we propose to align the difficulty of the generated patterns with the size of the synthetic dataset. In doing so, we successfully scale trajectory matching-based methods to larger synthetic datasets, achieving lossless dataset distillation for the very first time. Code and distilled datasets are available at https://gzyaftermath.github.io/DATM.

==> 8.check_list.tex <==
\section*{Checklist}

\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{} The improvement of BETA shrinks for the partial-set transfer task.
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{} See Sec.~\ref{sec:theory}.
        \item Did you include complete proofs of all theoretical results?
    \answerYes{} See the supplementary materials.
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{} Please refer to the supplementary materials.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} See Sec.~\ref{sec:exp-setting} and the supplementary materials.
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{} We report the average performance among three runs.
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)? See the supplementary materials.
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

==> macros.tex <==
\def\dc{\texttt{DC}}
\def\dsa{\texttt{DSA}}
\def\dm{\texttt{DM}}
\def\mtt{\texttt{MTT}}
\def\tesla{\texttt{TESLA}}

\algrenewcommand{\algorithmicrequire}{\textbf{Input:}}
\algrenewcommand{\algorithmicensure}{\textbf{Output:}}

==> tables/ablation-visda.tex <==
\begin{table}[!h]
\centering
\caption{\textcolor{black}{Ablation study of four learning objectives on VisDA-17.}}\label{tab:ablation-visda}
\scalebox{0.7}{
\begin{tabular}{l|cccccccccccc|c}
\toprule
Task & plane & bcycl & bus  & car  & horse & knife & mcycle & person & plant & sktbrd & train & truck & Per-class \\ \midrule
Source-only                    & 64.3  & 24.6  & 47.9 & 75.3 & 69.6  & 8.5   & 79.0   & 31.6   & 64.4  & 31.0   & 81.4  & 9.2   & 48.9      \\
$\mathcal{L}_{kd}$                       & 67.9  & 66.2  & 71.4 & 85.9 & 77.6  & 0.0   & 64.4   & 60.8   & 86.1  & 71.4   & 87.7  & 22.9  & 63.5      \\
$\mathcal{L}_{kd}+\mathcal{L}_{mi}$                & 81.4  & 86.7  & 77.9 & 55.1 & 92.2  & 34.6  & 80.8   & 79.9   & 87.3  & 87.9   & 84.3  & 58.7  & 75.6      \\
$\mathcal{L}_{dd}+\mathcal{L}_{mi}$                & 94.9  & 90.2  & 85.4 & 61.1 & 95.5  & 93.1  & 85     & 83.8   & 92.9  & 93.9   & 91.1  & 55    & 85.1      \\
$\mathcal{L}_{kd}+\mathcal{L}_{mi}+\mathcal{L}_{dd}$         & 94.8  & 84.1  & 79.9 & 70.1 & 94.3  & 83.7  & 83.3   & 82.8   & 92.4  & 88.6   & 88.2  & 45.4  & 82.3      \\
$\mathcal{L}_{kd}+\mathcal{L}_{mi}+\mathcal{L}_{dd}+\mathcal{L}_{adv}$ & 96.2  & 83.9  & 82.3 & 71.0 & 95.3  & 73.1  & 88.4   & 80.6   & 95.5  & 90.9   & 88.3  & 45.1  & 82.6   \\ \bottomrule  
\end{tabular}}
\end{table}

==> tables/ablation.tex <==

\begin{table}[]
\vspace{-1mm}
\caption{Ablation studies of learning objectives and MTN on Office-Home.}\label{tab:ablation}
\scriptsize
\resizebox{\columnwidth}{!}{
    \begin{tabular}{
    ccccc|cccccc
    >{\columncolor[HTML]{DAE8FC}}c}
    \toprule
    $\mathcal{L}_{dd}$ & $\mathcal{L}_{kd}$ & $\mathcal{L}_{mi}$ & $\mathcal{L}_{adv}$ & MTN          & Ar$\to$Cl & Cl$\to$Ar & Cl$\to$Pr & Pr$\to$Ar & Pr$\to$Cl & Re$\to$Cl & H. Avg. \\ \midrule
                       &                    &                    &                                       &              & 44.1  & 54.5  & 63.3  & 52.8  & 41.2  & 46.7  & 50.4    \\
    $\checkmark$       &                    &                    &                                       &              & 55.5  & 65.4  & 76.5  & 64.4  & 50.7  & 58.1  & 61.8    \\
    & $\checkmark$       &                    &                                       &              & 54.6  & 63.8  & 75.3  & 62.3  & 48.0    & 55.7  & 60.0    \\
    $\checkmark$       &                    &                    &                                       & $\checkmark$ & 56.6  & 65.0    & 76.7  & 64.1  & 51.6  & 60.4  & 62.4    \\
    $\checkmark$       &                    & $\checkmark$       &                                       & $\checkmark$ & 55.4  & 67.6  & 78.4  & 65.4  & 54.5  & 58.5  & 63.3    \\
    $\checkmark$       & $\checkmark$       & $\checkmark$       &                                       & $\checkmark$ & 56.8  & 68.1  & 78.7  & 67.3  & 55.3  & 59.2  & 64.2    \\
    $\checkmark$       & $\checkmark$       & $\checkmark$       & $\checkmark$                          & $\checkmark$ & 57.2  & 68.0  & 78.6  & 67.5  & 56.0  & 58.9  & 64.4   \\
    \bottomrule
    \end{tabular}
    }
    \vspace{-3mm}
\end{table}

==> tables/ablation_main.tex <==
\begin{table}[]
\centering
\scalebox{0.9}{
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{cccccc}
\toprule
Soft Label Initialization &     & \checkmark    & \checkmark    & \checkmark   & \checkmark \\
Sequential Arrangement    &     &     & \checkmark  & \checkmark  & \checkmark    \\
Soft Label Optimization   &     &     &     & \checkmark & \checkmark    \\
Difficulty Alignment      &     &     &  &      & \checkmark    \\ \midrule
Acc                       & 50.2 & crash & 50.7 & 52.0 & 53.3 \\ 
\bottomrule
\end{tabular}
}
\caption{Ablation study on CIFAR-100 with IPC=50, where ConvNetD3 is used for the distillation and evaluation.}
\label{tab: main ablation}
\end{table}

==> tables/comparison-dividemix.tex <==
\begin{table}[!h]
\centering
\caption{\textcolor{black}{The differences between our method and DivideMix.}}\label{tab:difference-dividemix}
\begin{tabular}{|p{2cm}|p{8cm}|p{3cm}|}\toprule
            & BETA                                 & DivideMix      \\ \midrule
Task        & Domain Adaptation of Black-box Predictior (DABP). the noise of the target domain in DABP is caused by domain shift between two different domains.   & Learning with Noisy Labels (LNL). The noise of LNL is randomly added.                     \\ \midrule
Method      & (a) BETA uses GMM to divide the target domain and MixMatch with different augmentation for semi-supervised learning. (similar) (b) BETA applies knowledge distillation between models in parallel to the semi-supervised learning, which is purified by the subdomain division to suppress error accumulation during distillation. (c) Subdomain alignment is proposed to align the internal domain shift. (d) Subdomain augmentation is proposed to enhance structural regularization (i.e., mutual information and mix-up). Strong-weak augmentation fully utilizes the high-confidence samples in $X_e$ and single weak augmentation does not introduce more noise to $X_h$. This process enhances the $L_{mi}$ in Eq.(8) that encourages the model to better comply with the cluster assumption and prevent the partiality for categories. & DivideMix uses GMM to divide the data and then use MixMatch for semi-supervised learning. \\ \midrule
Theory      & BETA analyzes the algorithm design theoretically and its connection with the learning shift of DABP.  A new bound of DABP is derived to explain the rationale behind the optimization.                                            & N.A.                                                                                      \\ \midrule
Experiments & Experiments on Office-Home demonstrate that BETA outperforms DivideMix by 4.7\% on average. For the hard tasks with distant domain shift, BETA outperforms DivideMix by 6.0\% on average.                          & Experiments are conducted on LNL benchmarks.    \\ \bottomrule                                         
\end{tabular}
\end{table}

